GenUDC: High Quality 3D Mesh Generation with Unsigned Dual Contouring Representation

Generating high-quality meshes with complex structures and realistic surfaces is the primary goal of 3D generative models. Existing methods typically employ sequence data or deformable tetrahedral grids for mesh generation. However, sequence-based methods have difficulty producing complex structures with many faces due to memory limits. The deformable tetrahedral grid-based method MeshDiffusion fails to recover realistic surfaces due to the inherent ambiguity in deformable grids. We propose the GenUDC framework to address these challenges by leveraging the Unsigned Dual Contouring (UDC) as the mesh representation. UDC discretizes a mesh in a regular grid and divides it into the face and vertex parts, recovering both complex structures and fine details. As a result, the one-to-one mapping between UDC and mesh resolves the ambiguity problem. In addition, GenUDC adopts a two-stage, coarse-to-fine generative process for 3D mesh generation. It first generates the face part as a rough shape and then the vertex part to craft a detailed shape. Extensive evaluations demonstrate the superiority of UDC as a mesh representation and the favorable performance of GenUDC in mesh generation. The code and trained models are available at https://github.com/TrepangCat/GenUDC.

==> caption/rebuttal_get3d.tex <==

\setlength{\abovecaptionskip}{-0mm}
\setlength{\belowcaptionskip}{-0mm}
\setlength{\textfloatsep}{-0mm}
\begin{figure}
    % \vspace{-0mm}
    \centering
    % \fbox{\rule{0pt}{2.5in} \rule{0.9\linewidth}{0pt}}\
    \includegraphics[width=\linewidth]{img/rebuttal_figure.pdf}
    % \vspace{-0mm}
    \caption{
    (a) Results of Get3D and ours. (b) Results of our method on vases in the ModelNet dataset.
    }
    % \vspace{-0mm}
    % \vspace{-30pt}
    \label{fig: rebuttal_get3d}
\end{figure}

==> sec/AC_lettet.tex <==
Dear Area Chair,

We are writing to request your attention to the review comments provided by Reviewer nfF4 on our submission #369 to ACMMM. This reviewer's comments are notably vague and do not provide necessary evidence or references. This lack of clarity violates the last point of ACMMM's Reviewer Best Practices.

We highly suspect that his reviews are rather hasty. For instance, his fourth comment, in fact, has the obvious answer in our paper. Additionally, the comments made in points 2, 3, and 5 are too general, for which a responsible reviewer should have provided either clear evidence or specific references/suggestions.

We have tried our best to resolve the questions raised by this reviewer in our rebuttal. But we still would like to request your reconsideration of Reviewer nfF4's comments. We believe that every submission to the renowned ACMMM deserves a more informed and detailed review.

Thank you very much for your time and kindness.

Best regards,

==> sec/Y_rebuttal_content.tex <==
\renewcommand{\thetable}{\Alph{table}}
\renewcommand{\thefigure}{\Alph{figure}}

As abbreviations, we refer to Reviewer \textbf{gNsr} as \FirstReviewer, Reviewer \textbf{nfF4} as \SecondReviewer, and Reviewer \textbf{AfTh} as \ThirdReviewer.
We thank the reviewers for their valuable comments.
% We are encouraged that the reviewers found that our method is \emph{novel} (\FirstReviewer,  \SecondReviewer, \ThirdReviewer) and \emph{clearly written} (\FirstReviewer).
% We are glad they found the paper is \emph{well written} (\ThirdReviewer) and \emph{easy to follow} (\FirstReviewer).
% Moreover, \FirstReviewer \ recognized our pioneering contribution.
We are encouraged that all reviewers acknowledge our technical contribution and superior performance for mesh generation.
% Moreover, \FirstReviewer \ recognized the merit and potential impact of the idea.
% \SecondReviewer \ and \ThirdReviewer \ acknowledge our novel and technical contributions.
% We will incorporate all feedback in the revision.
Below, we try to address their concerns.

\noindent \FirstReviewer \textbf{ - UDC's Adaptability:}
Theoretically, UDC can handle geometry like Chairs and Tables.
Considering that MeshDiffusion shows similar performance variations across the Car, Chair and Table categories, we think that the inherent insufficiency of the dataset causes the relatively low performance on Chair and Table.
Nevertheless, our GenUDC outperforms MeshDiffusion for Car and gets the best results in most metrics for Chair and Table.

\noindent \FirstReviewer \textbf{ - Comparision with Get3D:}
Our work is superior to MeshDiffusion, as shown in our paper. 
MeshDiffusion has already proved to be superior to Get3D.
So, we do not include the results of Get3D in our comparison.
For illustration, we show some results of Get3D and ours in \cref{fig: rebuttal_get3d} (a).
% According to Sec. F in the supplementary of MeshDiffusion, it outperforms Get3D in 3D generation. 
% So, we do not compare ours with Get3D as our method is superior to MeshDiffusion.
% However, we also present some visual results of Get3D and ours in \cref{fig: rebuttal_get3d}.



\noindent \SecondReviewer \textbf{ - Innovation in Generating Complex Structures and Realistic Surfaces:}
Balancing the generation of complex structures and realistic surfaces is an open issue. 
Existing methods mostly attempt to generate structures and surfaces simultaneously, but they struggle to ensure the quality of both.
For example, SDF-StyleGAN uses MC to ensure surface realness, but the generated results often have structural deficiencies (Fig. 15 of SDF-StyleGAN). 
Conversely, MeshDiffusion can generate complex structures, but its surfaces are often crumpled (our Fig. 7). 
In this paper, we exploit UDC's distinctive capability to represent an object's structure and surface separately but consistently. 
Based on UDC's unique nature, we propose a two-stage generative framework that generates complex structures and realistic surfaces separately. 
This enables a better balance between the generation of complex structures and realistic surfaces.
% The networks of existing methods lack the capability to generate complex structures.
% In contrast, we use the advanced LDM network with the special training protocol to produce rough shapes with complex structures.
% Table 2 can indirectly support our claim about generating complex structures.
% % The LDM's training protocol and capability allow the face part generation to produce rough shapes with complex structures.
% UDC can directly and accurately represent realistic surfaces of meshes, which is hard for most existing 3D representations.
% Thus, we can use the vertex part generation to adjust the vertex coordinates of rough shapes to produce realistic surfaces. 
% We do an ablation study of the vertex part generation in Sec. 4.4 of the main paper.

\noindent \SecondReviewer \textbf{ - Experimental Design and Analysis:}
To fairly evaluate the unconditional mesh generation quality, we follow MeshDiffusion's experiment protocol, which is the latest and most related work.
We do qualitative and quantitative experiments to compare ours with related works and do our best to provide analysis in Lines 549-568.
% Four metrics and three distances are considered in those experiments.
% The methods for comparison are representative works in 3D generation using different mesh representations. 
% In those methods, MeshDiffusion is one of the latest papers in mesh generation and can generate meshes directly.
% We do qualitative and quantitative experiments to compare ours with them.
% We even consider the influence of resolution on the performance.
% Those comprehensive experiments are acknowledged by \FirstReviewer \ and \ThirdReviewer.
% We also provide analysis in Lines 549-568.

\noindent \SecondReviewer \textbf{ - Dataset Selection:}
We agree that more datasets would surely increase the convincingness. 
Unfortunately, the ShapeNetCore (v1) dataset was the only dataset with a large number of samples available at submission for unconditional mesh generation evaluation.
% So, we follow this protocol and only use this dataset for experiments.
We select five categories in this dataset, as commonly done in the literature.
We think that this multi-category setting can alleviate the effect of bias.
% The comparison methods all use the ShapeNetCore (v1) dataset.
% For a fair and comprehensive comparison, we do experiments on five categories of this dataset.
% The multi-categories setting can alleviate the effect of bias.
We additionally show some results of our method on the ModelNet dataset in \cref{fig: rebuttal_get3d} (b).
But no comparison was made on other datasets because the authors of all the counterpart methods have reported results only on the ShapeNetCore dataset.

\input{caption/rebuttal_get3d}

\noindent \SecondReviewer \textbf{ - UDC's Advantages and Limitations:}
Thanks for the advice. 
We will summarize the following discussions that are scattered in our original manuscript.
Lines 311-312 and 366-367 mention that UDC can model both watertight and non-watertight meshes. 
Furthermore, Sec. 4.5 and Lines 159-162 show that UDC is faster and takes less memory in the data fitting process.
UDC can better model the shape as discussed in Lines 859-861. 
As discussed in Lines 865-866 of Sec. 5, UDC suffers from the non-manifold issue.
We also mention the memory problem of UDC in Lines 869.

\noindent \SecondReviewer \textbf{ - Discussion on Neural Rendering:}
Thanks for the comment. 
We have tried Neural Rendering and made the following observations.
(i) Neural rendering takes too much time and memory, and this cost is often unacceptable (Lines 802-803).
(ii) It leads to much information loss because it compresses the 3D shape into a 2D image. 
This information loss is responsible for the crumpled surfaces of MeshDiffusion's results (column 3 of Fig. 7).
(iii) UDC is incompatible with Neural Rendering since gradient-based
based optimization is ineffective for UDC (see Tab. 1 in FlexiCubes [59]).

\noindent \ThirdReviewer \textbf{ - Normalization of $\mathcal{F}$:}
Experimentally, we find that normalizing $\mathcal{F}$ to [-1.0, 1.0] can speed up the training process without sacrificing performance.

\noindent \ThirdReviewer \textbf{ - UDC vs. SDF:}
The relationship between SDF and mesh is one-to-many mapping depending on the employed post-processing.
% One SDF may correspond to multiple meshes depending on the different post-processing methods. 
UDC is free of such ambiguity.
Besides, UDC can explicitly model the shape details, while SDF only represents an obscure shape.

\noindent \ThirdReviewer \textbf{ - Generating Shapes with Different Orientations:}
For a convenient comparison of visualization, we render shapes in similar orientations, though they do have different orientations.

\noindent \ThirdReviewer \textbf{ - How Are Vertices Compatible with Faces?}
As discussed in Lines 340-343, the generated $\mathcal{V}$ can be seen as candidate vertices, and $\mathcal{F}$ determines which vertices make up the faces. 
Since each value of $\mathcal{F}$ is related to an edge of the grid, and each edge has four adjacent vertices, there would not be a mismatch or cases where a face cannot find its vertices.
The $\mathcal{F}$ values corresponding to boundary edges are meaningless and ignored.
Vertices that are not parts of faces are removed.
The remaining vertices and faces constitute the mesh.
This way, vertices are compatible with faces.

\noindent \ThirdReviewer \textbf{ - Generation Protocol:}
All the results are produced by unconditional generation, as is commonly done in the literature.
However, the diffusion model of LDM, which is employed to produce the input shape code of VAE, is trained in a category-specific manner (Lines 505-508).
For example, to generate a chair, we use the chair diffusion model to sample from the noise, synthesizing a shape code of the chair.
This shape code is then processed by VAE and U-Net to get the final chair mesh.
% Such a generation protocol is common in related works.

